Numerical Methods and Analysis of Computing Quasiperiodic Systems

Quasiperiodic systems are important space-filling ordered structures, without decay and translational invariance. How to solve quasiperiodic systems accurately and efficiently is of great challenge. A useful approach, the projection method (PM) [J. Comput. Phys., 256: 428, 2014], has been proposed to compute quasiperiodic systems. Various studies have demonstrated that the PM is an accurate and efficient method to solve quasiperiodic systems. However, there is a lack of theoretical analysis of PM. In this paper, we present a rigorous convergence analysis of the PM by establishing a mathematical framework of quasiperiodic functions and their high-dimensional periodic functions. We also give a theoretical analysis of quasiperiodic spectral method (QSM) based on this framework. Results demonstrate that PM and QSM both have exponential decay, and the QSM (PM) is a generalization of the periodic Fourier spectral (pseudo-spectral) method. Then we analyze the computational complexity of PM and QSM in calculating quasiperiodic systems. The PM can use fast Fourier transform, while the QSM cannot. Moreover, we investigate the accuracy and efficiency of PM, QSM and periodic approximation method in solving the linear time-dependent quasiperiodic Schr\"{o}dinger equation.

==> ex_shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.

% Packages and macros go here
\usepackage{mathrsfs,amsmath,amssymb,bm,subfigure,float,geometry}
\usepackage{booktabs,mathtools,algorithm}
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{epstopdf}
\usepackage{makecell, rotating}
\usepackage{multirow}
\usepackage{algorithmic}
\usepackage{ntheorem}
%\usepackage{estin}
\usepackage{tikz}
\newcommand{\averageint}{
    \mbox{
        \tikz[baseline = (int.base)] { \node (int) {$\int$}; \node at (int) {$-$}; }
    }
}


\usepackage{indentfirst}
\setlength{\parindent}{2em}
%\usepackage[table,xcdraw]{xcolor}
%\usepackage[table,xcdraw]{xcolor}

\usepackage[ulem={normalem,normalbf}]{changes}
%\definechangesauthor[name={Kai Jiang},color=violet]{jk}
%\definechangesauthor[name={Kai Jiang}, color=red]{jk}
% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}
\newcommand{\by}{\bm{y}}
\newcommand{\bz}{\bm{z}}
\newcommand{\bx}{\bm{x}}
\newcommand{\bp}{\bm{p}}
\newcommand{\tbx}{\tilde{\bm{x}}}
\newcommand{\tdP}{\tilde{\bm{P}}}
\newcommand{\tdQ}{\tilde{\bm{Q}}}
\newcommand{\ba}{\bm{a}}
\newcommand{\bb}{\bm{b}}
\newcommand{\be}{\bm{e}}
\newcommand{\bn}{\bm{n}}
\newcommand{\br}{\bm{r}}
\newcommand{\bh}{\bm{h}}
\newcommand{\bH}{\bm{H}}
\newcommand{\bN}{\bm{N}}
\newcommand{\bk}{\bm{k}}
\newcommand{\bj}{\bm{j}}
\newcommand{\bv}{\bm{v}}
\newcommand{\bV}{\bm{V}}
\newcommand{\vbk}{\bm{k}}
\newcommand{\vbw}{\bm{w}}
\newcommand{\vbv}{\bm{v}}

\newcommand{\DbV}{\Delta \bm{V}}
\newcommand{\bw}{\bm{w}}
\newcommand{\bW}{\bm{W}}
\newcommand{\bo}{\bm{0}}
\newcommand{\bR}{\bm{R}}
\newcommand{\bO}{\bm{O}}
\newcommand{\bhphi}{\bm{\hat{\phi}}}
\newcommand{\bhpsi}{\bm{\hat{\psi}}}
\newcommand{\bphi}{\bm{{\phi}}}
\newcommand{\bt}{\bm{t}}
\newcommand{\bs}{\bm{s}}
\newcommand{\bu}{\bm{u}}
\newcommand{\bM}{\bm{M}}
\newcommand{\bP}{\bm{P}}
\newcommand{\bQ}{\bm{Q}}
\newcommand{\bB}{\bm{B}}
\newcommand{\bA}{\bm{A}}
\newcommand{\bI}{\bm{I}}
\newcommand{\bmm}{\bm{m}}
\newcommand{\bell}{\bm{\ell}}
\newcommand{\btau}{\bm{\tau}}
\newcommand{\blam}{\bm{\lambda}}
\newcommand{\bLam}{\bm{\Lambda}}
\newcommand{\ellinf}{\ell^{\infty}}
\newcommand{\tilvarepsilon}{\tilde{\varepsilon}}
\newcommand{\tilalpha}{\tilde{\alpha}}
\newcommand{\hatvarphi}{\hat{\varphi}}
\newcommand{\tilvarphi}{\tilde{\varphi}}
\newcommand{\hatblam}{\hat{\bm \lambda}}

\newcommand{\bbR}{\mathbb{R}}
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbZ}{\mathbb{Z}}
\newcommand{\bbQ}{\mathbb{Q}}
\newcommand{\bbM}{\mathbb{M}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbX}{\mathbb{X}}
\newcommand{\bbT}{\mathbb{T}}
\newcommand{\bbc}{\mathbb{c}}
\newcommand{\bbs}{\mathbb{s}}

\newcommand{\calC}{\mathcal{C}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\cala}{\mathcal{a}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\hF}{\hat{F}}
\newcommand{\hc}{\hat{c}}
\newcommand{\bq}{\bm{q}}
\newcommand{\hw}{\hat{w}}
\newcommand{\hphi}{\hat{\phi}}
\newcommand{\hPhi}{\hat{\Phi}}
\newcommand{\hpsi}{\hat{\psi}}
\newcommand{\hPsi}{\hat{\Psi}}
\newcommand{\hxi}{\hat{\xi}}
\newcommand{\hJ}{\hat{J}}
\newcommand{\hu}{\hat{u}}
\newcommand{\hf}{\hat{f}}
\newcommand{\vzero}{\bm{0}}
\newcommand{\tE}{\tilde{E}}
\newcommand{\tF}{\tilde{F}}
\newcommand{\tf}{\tilde{f}}
\newcommand{\tG}{\tilde{G}}
\newcommand{\tg}{\tilde{g}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\bg}{\bar{g}}
\newcommand{\tJ}{\tilde{\mathcal{J}}}
\newcommand{\td}{\tilde{d}}
\newcommand{\la}{\langle}
\newcommand{\ra}{\rangle}
\newcommand{\dom}{\mathrm{dom}}
\newcommand{\spar}{\scriptscriptstyle{\|}}
\newcommand{\sperp}{\scriptscriptstyle{\perp}}
\DeclareMathOperator{\intdom}{\mathrm{int}\dom}
\DeclareMathOperator{\ridom}{\mathrm{ri}\dom}
\DeclareMathOperator{\affdom}{\mathrm{aff}\dom}
\newcommand{\recheck}[1]{{\color{red}{#1}}}
%\newcommand{\avint}{\mathop{\ooalign{$\int$\cr$-$}}}

\newcommand{\inner}[1]{\left<#1\right>_{AP}}
\newcommand{\norm}[1]{\left\|#1\right\|^{2}_{AP}}

\newcommand{\Tri}{\mbox{Tri}}
\newcommand{\QP}{\mbox{QP}}

\newtheorem*{proof}{Proof}
\newtheorem{thm}{Theorem}[section]
\newtheorem{lemma}[thm]{Lemma}
\newtheorem{proposition}[thm]{Proposition}
\newtheorem{corollary}[thm]{Corollary}
\newtheorem{defy}[thm]{Definition}
\newtheorem{remark}[thm]{Remark}
\newtheorem{example}[thm]{Example}
\newtheorem{assumption}[thm]{Assumption}
\newtheorem{prop}[thm]{Properties}

\newcommand\tbbint{{-\mkern -16mu\int}}
\newcommand\tbint{{\mathchar '26\mkern -14mu\int}}
\newcommand\dbbint{{-\mkern -19mu\int}}
\newcommand\dbint{{\mathchar '26\mkern -18mu\int}}
\newcommand\bint{
	{\mathchoice{\dbint}{\tbint}{\tbint}{\tbint}}
}
\newcommand\bbint{
	{\mathchoice{\dbbint}{\tbbint}{\tbbint}{\tbbint}}
}

\allowdisplaybreaks[4]
\DeclareMathOperator*{\argmin}{\mathrm{argmin}}
\DeclareMathOperator*{\argmax}{\mathrm{argmax}}

\newcommand{\Prox}{\mathrm{Prox}}
\newcommand{\BProx}{\mathrm{BProx}}
\newcommand{\GProx}{\mathrm{GProx}}
\newcommand{\dist}{\mathrm{dist}}
%\newcommand{\mod}{\mathrm{mod}}

%\renewcommand{\baselinestretch}{1.5}


%% Used for creating new theorem and remark environments
%%\newsiamremark{remark}{Remark}
%\newsiamremark{hypothesis}{Hypothesis}
%\crefname{hypothesis}{Hypothesis}{Hypotheses}
%\newsiamthm{claim}{Claim}
%
%% Sets running headers as well as PDF title and authors
%\headers{Title}{Authors.}
%
%% Title. If the supplement option is on, then "Supplementary Material"
%% is automatically inserted before the title.
%\title{Analysis of the numerical method for quasicrystals
%     }
%
%% Authors: full names plus addresses.
%\author{Kai Jiang
%%	\thanks{Imagination Corp., Chicago, IL
%%  (\email{ddoe@imag.com}, \url{http://www.imag.com/\string~ddoe/}).}
%}
%
%\usepackage{amsopn}
%\DeclareMathOperator{\diag}{diag}
%
%
%%% Added on Overleaf: enabling xr
%\makeatletter
%\newcommand*{\addFileDependency}[1]{% argument=file name and extension
%  \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
%  \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
%  \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
%}
%\makeatother
%
%\newcommand*{\myexternaldocument}[1]{%
%    \externaldocument{#1}%
%    \addFileDependency{#1.tex}%
%    \addFileDependency{#1.aux}%
%}
%%%% END HELPER CODE
%%%% Local Variables:
%%%% mode:latex
%%%% TeX-master: "ex_article"
%%%% End:

